Search for Gravitational Waves from Compact Binary Coalescence in LIGO and Virgo Data from S5 and VSR1

We report the results of the first search for gravitational waves from compact binary coalescence using data from the LIGO and Virgo detectors. Five months of data were collected during the concurrent S5 (LIGO) and VSR1 (Virgo) science runs. The search focused on signals from binary mergers with a total mass between 2 and 35 Msun. No gravitational waves are identified. The cumulative 90%-confidence upper limits on the rate of compact binary coalescence are calculated for non-spinning binary neutron stars, black hole-neutron star systems, and binary black holes to be 8.7x10^-3, 2.2x10^-3 and 4.4x10^-4 yr^-1 L_10^-1 respectively, where L_10 is 10^10 times the blue solar luminosity. These upper limits are compared with astrophysical expectations.

==> Makefile <==
SHELL=/bin/sh

PROJECT=s5-2yr-ligovirgo-lowcbc
TEXFILES=s5-2yr-ligovirgo-lowcbc.tex
BIBTEXFILES=../bibtex/iulpapers.bib
PUBLISHFILES=
EXTRA_DIST=

TEXFLAGS=-interaction=batchmode
LATEX=latex $(TEXFLAGS)
DVIPS=dvips
DVIPDF=dvipdf
PDFLATEX=pdflatex
BIBTEX=bibtex
TAR=tar
DISTFILES= s5-2yr-ligovirgo-lowcbc.tex authorlist.tex iulpapers.bib ./Images/*eps ./Images/*.png Makefile

all: pdf

publish: $(TEXFILES) $(BIBTEXFILES) pat
	./publish.sh
	for file in  publish.tex  ; do \
	  base=`basename $$file .tex`; \
          $(PDFLATEX) $$base && \
	  $(PDFLATEX) $$base ;  \
	done
	mkdir pubtmp
	for file in "s3s4.tex" ; do \
	  cp $$file ./pubtmp/ ; \
	done
	cd pubtmp ; \
	tar -zcvf ../publish.tar.gz ./*


dvi: $(TEXFILES) $(BIBTEXFILES)
	for file in $(TEXFILES) ; do \
	  base=`basename $$file .tex`; \
          $(LATEX)  $$base && \
	  $(BIBTEX) $$base && \
	  $(LATEX)  $$base && \
	  $(LATEX)  $$base ;  \
	done

ps: dvi
	for file in $(TEXFILES) ; do \
	  base=`basename $$file .tex`; \
          $(DVIPS) $$base -o ; \
	done

pdf: $(TEXFILES) $(BIBTEXFILES)
	for file in $(TEXFILES) ; do \
	  base=`basename $$file .tex`; \
          $(PDFLATEX) $$base && \
	  $(BIBTEX)   $$base && \
	  $(PDFLATEX) $$base && \
	  $(PDFLATEX) $$base ;  \
	done

dist:
	if test -d dist ; then rm -fr dist; fi ; \
	mkdir dist ; \
	for file in $(DISTFILES) ; do cp $$file dist ; done ; \
	$(TAR) chozf dist.tar.gz dist ; \
	rm -fr dist

clean:
	for file in $(TEXFILES) ; do \
	  base=`basename $$file .tex` ; \
          rm -f $$base.log $$base.aux $$base.end $$base.bbl $$base.blg; \
	done

realclean: clean
	for file in $(TEXFILES) ; do \
	  base=`basename $$file .tex` ; \
          rm -f $$base.ps $$base.dvi $$base.pdf; \
	done
	rm -f publish.tex publish.aux publish.dvi publish.pdf publish.log
	rm -f top.tex body.tex
	rm -rf pubtmp

